VisionLLM v2: An End-to-End Generalist Multimodal Large Language Model for Hundreds of Vision-Language Tasks

We present VisionLLM v2, an end-to-end generalist multimodal large model (MLLM) that unifies visual perception, understanding, and generation within a single framework. Unlike traditional MLLMs limited to text output, VisionLLM v2 significantly broadens its application scope. It excels not only in conventional visual question answering (VQA) but also in open-ended, cross-domain vision tasks such as object localization, pose estimation, and image generation and editing. To this end, we propose a new information transmission mechanism termed "super link", as a medium to connect MLLM with task-specific decoders. It not only allows flexible transmission of task information and gradient feedback between the MLLM and multiple downstream decoders but also effectively resolves training conflicts in multi-tasking scenarios. In addition, to support the diverse range of tasks, we carefully collected and combed training data from hundreds of public vision and vision-language tasks. In this way, our model can be joint-trained end-to-end on hundreds of vision language tasks and generalize to these tasks using a set of shared parameters through different user prompts, achieving performance comparable to task-specific models. We believe VisionLLM v2 will offer a new perspective on the generalization of MLLMs.

==> tables/region_cap.tex <==
\begin{table*}[t!]
\scriptsize
\centering

\setlength\tabcolsep{2pt}
\renewcommand{\arraystretch}{1.2}



\begin{tabular}{l|cc|cc|cc}
           & \multicolumn{2}{c|}{RefCOCOg} & \multicolumn{2}{c|}{VG (full set)} & \multicolumn{2}{c}{VG (subset)} \\
        \multirow{-2}{*}{method} & METEOR & CIDEr & METEOR & CIDEr & METEOR & CIDEr  \\

    \hline
    GRiT~\cite{wu2022grit} & 15.2 & 71.6 & 17.1 & 142.0 & - & - \\
    Kosmos-2~\cite{peng2023kosmos2} & 14.1 & 62.3 & - & - & - & - \\
    GPT4RoI~\cite{zhang2023gpt4roi} & - & - & 17.4 & 145.2 & - & - \\
    ASM~\cite{wang2023allseeing} & 20.8 & 103.0 & 18.0 & 145.1 & - & -\\
    RegionGPT~\cite{guo2024regiongpt} & 16.9 & 109.9 & 17.0 & 145.6 & - & - \\
    PixelLLM~\cite{xu2023pixelllm} & 14.3 & 82.3 & 19.9 & 148.9 & - & - \\
    GLaMM~\cite{rasheed2023glamm} & 16.1 & 107.3 & - & - & 19.0 & 163.9 \\
    Groma~\cite{ma2024groma} & 16.8 & 107.3 & - & - & 19.0 & 158.4 \\

    \hline
    \rowcolor{gray!15}
    \modelname-Chat & 21.2 & 118.5 & 17.8 & 149.2 & 20.0 & 172.3 \\
    \rowcolor{gray!15}
    \modelname & 20.4 & 111.6 & 16.4 & 131.9 & 18.8 & 156.9 \\

\end{tabular}


\caption{\textbf{Comparison of region captioning performance.} 
% Zero-shot image captioning is evaluated on Flickr30K test set~\cite{plummer2015flickr30k} and NoCaps validation set~\cite{agrawal2019nocaps}, using CIDEr as evaluation metric. 
For region captioning on Visual Genome~\cite{krishna2017visual}, full set refers to the use of all validation samples for evaluation, while subset denotes the 5000 samples specified by~\cite{rasheed2023glamm}.
}
\label{tab:region_cap}
\end{table*}
